Conversation Modeling on Reddit using a Graph-Structured LSTM

This paper presents a novel approach for modeling threaded discussions on social media using a graph-structured bidirectional LSTM which represents both hierarchical and temporal conversation structure. In experiments with a task of predicting popularity of comments in Reddit discussions, the proposed model outperforms a node-independent architecture for different sets of input features. Analyses show a benefit to the model over the full course of the discussion, improving detection in both early and late stages. Further, the use of language cues with the bidirectional tree state updates helps with identifying controversial comments.

==> conclusion.tex <==
\section{Related work}
\label{sec:literature}

Popularity prediction task, which also can be referred as community endorsement, gaining attention across different social media platforms. An approximation for popularity can refer to either posts or comments, and can range from a number of shares on Facebook \cite{cheng2014can} and Twitter \cite{bandari2012pulse}, number of retwitts \cite{tan2014effect,zhao2015seismic,bi2016modeling} and difference in number of upvotes and downvotes on Reddit \cite{lakkaraju2013s,jaech2015talking,fang2016learning}. Popularity prediction is a hard task where lots of factors can play a role, that is why most of prior studies would control for factors such as topic \cite{tan2014effect,weninger2013exploration}, timing information \cite{tan2014effect,jaech2015talking}, comment content \cite{lakkaraju2013s} or graph representation \cite{jaech2015talking}. Controlling for some of the factors is convenient in understanding some components of successful post, but does not allow to use such algorithms in a real world scenarios. \cite{fang2016learning} and \cite{bi2016modeling} attempted in predicting the popularity without controlling for any of the factors on Reddit and Twitter correspondingly. In our study we are also interested in popularity prediction in a more general real life setting with no restriction to specific factors. Our work is close to \cite{fang2016learning} from the task prospective. We are using the same task of quantized karma prediction on Reddit and share some of the metrics, where we do not control for any of the factors and process the whole thread as is. The main difference of our work to \cite{fang2016learning} is that here we represent the whole conversation thread in a single global model in opposed to using only a local information based on the feature representation.

Tree-RNNs, with the most popular tree-LSTMs, are recent modification of a conventional sequential RNN and used in a verity of NLP tasks with a primarily goal of sentence modeling \cite{tai2015improved,zhu2015long,zhang2016top}. The architecture of tree-RNNs varies and primarily depends on the task, where the task dictates a number of children and their relationship in the tree. Some options include summarizing over the children, adding a separate forget gate for each of the child \cite{tai2015improved}, or recurrent propagation among siblings \cite{zhang2016top}. To the best of out knowledge our work is the first that uses tree-LSTM to model a conversation in opposed to a single sentence. Also, different to prior works, our architecture concurrently incorporates two different recursive prospectives in one LSTM unit - hierarchical and timing.

\section{Conclusion}

In this paper we present a novel approach for modeling conversations on social media using graph-structured LSTM. We study the importance of a global representation of the thread using the popularity prediction task on Reddit, where we compare our approach to a node-independent architecture using local set of submission context features. While we evaluate our model on predicting the popularity of comments in Reddit, our model is general enough and can be applied to various of problems and domains. Such domains can include additional subreddits, or other social media platforms such as Twitter, Facebook. Possible tasks may include popularity prediction, influence detection or other tasks that would require a truck of conversation dynamics such as topic or opinion shifts.
Our analysis show that our global model is better in predicting challenging comments including popular comments that are further away from the original post or posted later in the discussion. In addition, we study the importance of language representation in popularity prediction task. Our findings suggest that language plays a very important for popularity prediction especially in some specific types of the comments including jokes and controversial comments.

Since current approach uses a very simplistic representation of textual information one of the main direction of our future work is to concentrate on a better representation of the comment content. Possible architectures for representing the language of the comment include attention-based RNN and convolutional architectures to capture the topic and style of the conversation. Also, based on the analysis of using textual information, one of the interesting directions of the future work would be to improve an automatic prediction of jokes and funny comments. In addition, we are interested to improve the pruning step with a more sofisticated yet simple classifier that can take into account a textual information in order to improve the performance for \textit{unerpredicted} comments.

==> intro.tex <==
\section{Introduction}

Social media is a convenient platform for interactions and discussions among users. Often, those conversations presented in a tree structure where comments represent nodes, the root is the original post, and each new reply to any of the previous comments added as a leaf to the correspondent comment. Some examples of the most popular services with tree-like structure include Facebook, Reddit, Quora, and StackExchange. Figure \ref{fig: visual} shows an example conversation on Reddit, where bigger nodes associate with the higher upvoted comments\footnote{The visualization was obtained by using https://whichlight.github.io/reddit-network-vis}. Alternatively, in some services like Twitter tweets and their retweets can also be viewed as forming a tree structure. Having a tree structure allows the user to see partial or whole history of the conversation up to some point, and respond to the most interesting part of it. That is why modeling and viewing the conversation as a whole allows a better understanding of the content and dynamics of the discussion.

\begin{figure}[t]
\centering
\includegraphics[scale=0.35]{tree_example.png}
\caption{Visualization of a sample thread on Reddit.}
\label{fig: visual}
\end{figure}

\begin{figure*}[t]
\centering
\subfigure[Forward hierarchical structure]{\label{fig:a}
\includegraphics[scale=0.5]{forward_hierarchical_lstm.png}} \qquad
\subfigure[Forward timing structure]{\label{fig:b}
\includegraphics[scale=0.5]{forward_time_lstm.png}} \qquad
\subfigure[Backward hierarchical and timing structure]{\label{fig:c}
\includegraphics[scale=0.5]{backward_lstm.png}} \qquad

\caption{An example of model propagation in a graph-structured LSTM. Here, the node name are shown in a chronological order, e.g. comment $t1$ was made earlier than $t2$.\ref{fig:a} Hierarchical propagation of LSTM in the forward direction. \ref{fig:b} Timing propagation of LSTM in forward direction. \ref{fig:c} Backward propagation of tree-LSTM. Blue arrows represent hierarchical propagation, green arrows represent timing propagation.}
\label{lstm_example}
\end{figure*}

One interesting task in social media is popularity prediction, which is also sometimes referred as community endorsement. Often, each comment is associated with a score dependent on a number of upvotes/likes and downvotes/dislikes. The task would be to predict which comments associated with the high vs low scores. Previous studies found that time when the comment/post was published has a huge impact on its popularity \cite{lakkaraju2013s,jaech2015talking}. In addition, graph cues can be predictive of the popularity. For example, a high number of replies to the comment can often be an indicator of its popularity, although some comments with a high number of replies can be either controversial or have a highly negative score. In those cases, the role of language can be extremely important. 

Previous studies suggest that learning the language cues associated with the popularity based on the whole conversation can be hard due to the dominance of time, topic and others factors \cite{lakkaraju2013s,tan2014effect}. Thus, previously authors usually constrained the problem to reduce the effect of those factors. On the other hand, predicting popularity in the original problem allows a better understanding of the global interest in the community and better use of such system in a real-world scenarios. In our study, we are interested in popularity prediction when reactions in terms of graph and time features are fully known.


In this paper, we introduce a novel approach of modeling a whole conversation using a single graph-structured LSTM, where each comment in the tree corresponds to a single LSTM unit. 
%Our approach allows to automatically track the dynamics of the conversation such as shifts in topic or attention, thus allowing a better global representation of the problem. 
For example, modeling each comment separately using a set of features allows limited amount information about other popular comments in a discussion. Having an additional information about other potentially very successful comments made previously allows the model to modify the predicted score accordingly.  
%While we evaluate our model on predicting the popularity of comments in Reddit forum discussions, our model is general enough and can be applied to various of problems and domains. 

%%MO: need to work this in
In popularity prediction task, both graph structure and timing are extremely important. That is why in our tree structured LSTM we model the problem from two prospectives - hierarchical and timing.

The main contributions of this paper include: (a) a novel approach for conversation modeling in social media; (b) evaluation of the model in the popularity prediction task on Reddit; (c) analysis of the capabilities of the model including the importance of language representation.


==> method.tex <==
\section{Method}
\label{method}

\subsection{Graph-structured LSTM for thread modeling}

Our model is a global bidirectional tree-LSTM that corresponds to a single thread. In this paper, we will refer to this model as a graph-structured model. Here each comment in a conversation, or each node in a tree, represented by a single LSTM unit. In popularity prediction task, both graph structure and timing are extremely important. That is why in our tree structured LSTM we model the problem from two prospectives - hierarchical and timing. Figures \ref{fig:a},\ref{fig:b} shows an example of the hidden states connection in hierarchical and timing structures for the forward LSTM. In a forward hierarchical structure, we pass the hidden states of LSTM from a parent to each of its children. In a timing structure, we pass the hidden states from the earlier comment to the later among the siblings. 
Here, our motivation and underlying assumption are that a user who decides on where to post looks mostly in a local context within the subtree, since often the whole tree can be very large and not observable by the user.

Our input in each state is a comment embedding, which can be modeled in various of ways. In this preliminary study, we use a bag-of-words representation for text with additional concatenated graph and time features. 
We slightly modify LSTM unit in order to include both hierarchical and timing structures for each comment. Specifically, we use two forget gates - one for previous hierarchical layer, and one for previous timing layer. Below is the set of equations describing LSTM unit, where $t-1$ denotes a timely previous layers, and $d-1$ denotes a hierarchically previous layers, $\sigma$ is a sigmoid function: 

\begin{equation}
\label{eq: 1}
\begin{aligned}
i_{t} &= \sigma(W_{i}x_{t} + U_{i}h_{t-1}  + W_{i}h_{d-1} + b_{i}) \\
f_t &= \sigma(W_{f}x_{t} + U_{f}h_{t-1} +W_{f}h_{d-1} + b_{f}) \\
g_t &= \sigma(W_{f}x_{t} + U_{f}h_{t-1} +W_{f}h_{d-1} + b_{f}) \\
\tilde{c}_{t} &= W_{c}x_{t} + U_{c}h_{t-1} + W_{c}h_{d-1} + b_{c} \\
c_t &= f_t * c_{t-1} + g_t * c_{d-1} + i_t * \tilde{c}_t \\
o_t &= \sigma(W_{o}x_{t} + U_{o}h_{t-1} +  W_{o}h_{d-1} + b_{o}) \\
h_t &= o_t * tanh( c_t)
\end{aligned}
\end{equation}

Assuming that the whole tree structure is known, at each state, we would like to have a complete information about the whole tree, since both earlier/upper and later/lower comments can be useful in determining the node's label. Similarly to the forward LSTM, we define a backward LSTM in the opposite direction with the only difference that in hierarchical structure only the earliest node will pass the hidden state to its parent. Figure \ref{fig:c} shows an example of both hierarchical and timing backward propagation.
 
Often the number of comments in a single subtree can be large, which makes it harder to train such a big network. Usually, only a very small part of the comments in conversation would have higher scores, while the majority of the comments will not get any attention at all. Having a preprocessing step that will allow us to prune at least part of unpopular comments will greatly decrease the computation cost. Here we will refer to such preprocessing step as pruning. On the other hand, those comments may still carry a useful information regarding the popularity of other comments. For example, a comment can have a high score while all its numerous children are pruned. In order to include the information from the pruned comments, we replace LSTM unit that corresponds to a pruned comment with a bias vector that learned during the training. We add biases for each of pruned comments to the next non-pruned hidden state. We include separate bias vectors in each direction for both hierarchical and timing structures, propagated in a way similar to our main architecture.

On top of LSTM unit we place a softmax layer over 8 quantized karma levels. Our objective function is a cross-entropy over the quantized levels, which described in more detail in Section ~\ref{sec: levels}. 

\subsection{Features}

\subsubsection{Baseline}

Our baseline includes the following features:

\textit{Time}: time since root, time since parent

\textit{Author}: if the author is the author of original post, number of comments made by the author in the conversation

\textit{Graph}: depth of the comment,  number of children, number of later comments, a number of previous comments, a number of siblings, subtree height, subtree size, a number of children normalized for each post, subtree size normalized for each post.  

All of the features above are represented as a vector and used as an input to the tree-LSTM unit. We will refer to this set of features as graph and time features.

\subsubsection{Language features}

 In addition to our baseline without any linguistic information, we also experiment with using a language of the comments and post to improve popularity prediction. In this preliminary study, each comment or post is modeled using a simple bag-of-words representation learned during the training for the up to 100 first words in the comment. Then, we concatenate the resulting language representation vector with our baseline features and use the resulting vector as an input. In all our experiments, we use bag-of-words embeddings with the dimension of 100 and restrict the vocabulary to include only the words that occurred at least 10 times in the dataset. In our future work, we are planning to extend the current simplistic text representation to a more complex one with a better fit for the task.
